Faster O(|V|^2|E|W)-Time Energy Algorithms for Optimal Strategy Synthesis in Mean Payoff Games

This study strengthens the links between Mean Payoff Games (\MPG{s}) and Energy Games (EG{s}). Firstly, we offer a faster $O(|V|^2|E|W)$ pseudo-polynomial time and $\Theta(|V|+|E|)$ space deterministic algorithm for solving the Value Problem and Optimal Strategy Synthesis in \MPG{s}. This improves the best previously known estimates on the pseudo-polynomial time complexity to: \[ O(|E|\log |V|) + \Theta\Big(\sum_{v\in V}\texttt{deg}_{\Gamma}(v)\cdot\ell_{\Gamma}(v)\Big) = O(|V|^2|E|W), \] where $\ell_{\Gamma}(v)$ counts the number of times that a certain energy-lifting operator $\delta(\cdot, v)$ is applied to any $v\in V$, along a certain sequence of Value-Iterations on reweighted \EG{s}; and $\texttt{deg}_{\Gamma}(v)$ is the degree of $v$. This improves significantly over a previously known pseudo-polynomial time estimate, i.e. $\Theta\big(|V|^2|E|W + \sum_{v\in V}\texttt{deg}_{\Gamma}(v)\cdot\ell_{\Gamma}(v)\big)$ \citep{CR15, CR16}, as the pseudo-polynomiality is now confined to depend solely on $\ell_\Gamma$. Secondly, we further explore on the relationship between Optimal Positional Strategies (OPSs) in \MPG{s} and Small Energy-Progress Measures (SEPMs) in reweighted \EG{s}. It is observed that the space of all OPSs, $\texttt{opt}_{\Gamma}\Sigma^M_0$, admits a unique complete decomposition in terms of extremal-SEPM{s} in reweighted EG{s}. This points out what we called the "Energy-Lattice $\mathcal{X}^*_{\Gamma}$ associated to $\texttt{opt}_{\Gamma}\Sigma^M_0$". Finally, it is offered a pseudo-polynomial total-time recursive procedure for enumerating (w/o repetitions) all the elements of $\mathcal{X}^*_{\Gamma}$, and for computing the corresponding partitioning of $\texttt{opt}_{\Gamma}\Sigma^M_0$.

==> Omitted-Proofs.tex <==
\subsection{Proof of Lemma~\ref{lem:ei-jump_state}}\label{subsect:ei-jump_increases_i}

\subsection{Proof of Proposition~\ref{prop:saint_weak_coherency_holds}}\label{subsect:proof_saint_weak_coherency_holds}
\begin{proof}[Proof of Proposition~\ref{prop:saint_weak_coherency_holds}]
The proof of Proposition~\ref{prop:saint_weak_coherency_holds} goes by induction on the number of invocations of 
$\texttt{J-VI}()$ (SubProcedure~\ref{algo:j-value-iteration}) that are made  
either at line~\ref{algo:jvalue:l12} of Algorithm~\ref{algo:solve_mpg} or 
at line~\ref{subproc:ua-jumps:l3} of $\texttt{ua-jumps}()$ (SubProcedure~\ref{subproc:ua-jumps}). 

\emph{Base Case.}
At the beginning of Algorithm~\ref{algo:solve_mpg}, $i=W^-$ and $j=1$ (see line~\ref{algo:solve:l6}).
So, the 1-th invocation of $\texttt{ei-jump}()$ (line~\ref{algo:solve:l8}) is made on input $(W^-, 1, \J)$.
Recall how $\texttt{ei-jump}()$ (SubProcedure~\ref{subproc:energy_jumps}) works. 
Since, $L^{\text{inc}}=\emptyset$ and $L_{\text{\bf{w}}}\neq\emptyset$ 
(as $\texttt{init\_jumper}()$ initialized them at line~\ref{algo:solve:l5} 
of Algorithm~\ref{algo:solve_mpg} and  lines~\ref{proc:jumper_init:l1}-\ref{proc:jumper_init:l2} 
of SubProcedure~\ref{proc:jumper_init}), it enters the \texttt{while} 
loop at line~\ref{subproc:energy_jump:l3} of $\texttt{ei-jump}()$ 
(SubProcedure~\ref{subproc:energy_jumps}). There inside, the front element $(W^-,L_{\alpha})$ of 
$L_{\text{\bf{w}}}$ is firstly popped (line~\ref{subproc:energy_jump:l4}), 
then $\J.i\leftarrow W^-$ is assigned (line~\ref{subproc:energy_jump:l5}), 
and $\texttt{repair}()$ is invoked on input $(L_{\alpha},\J)$ (line~\ref{subproc:energy_jump:l6}), 
notice $L_{\alpha}=\{e\in E\mid w_e=W^{-}\}$. For each $(u,v,W^-)\in L_{\alpha}$, 
since $\J.f[u]=0$ and $\J.f[v]=0$ (as initialized by $\texttt{init\_jumper}()$), and since 
$L^{\text{inc}}[u]=\bot$ (because $L^{\text{inc}}$ was initialized to be empty by $\texttt{init\_jumper}()$), 
then $(u,v)\in E$ is (correctly) recognized as an incompatible arc at line~\ref{subproc:repair:l2} of $\texttt{repair}()$; 
this is correct because $i=W^-$, $j=1$, $w(u,v)=W^-$, and $f^{\text{c}}(u)=f^{\text{c}}(v)=0$, so  
$(u,v)$ is really incompatible with respect to $f^{\text{c}}=\bf{0}$ in $\Gamma_{i,j}=\Gamma_{W^-,1}$.
As such, if $u\in V_1$, then $u$ is (correctly) inserted into $L^{\text{inc}}$ (line~\ref{subproc:repair:l3} 
of $\texttt{repair}()$); else, $u\in V_0$, thus, 
$\J.\texttt{cnt}[u]$ is (correctly) decremented by one unit (line~\ref{subproc:repair:l5}), 
and it is (correctly) assigned $\J.\texttt{inc}[(u,v)]\leftarrow\texttt{true}$ (line~\ref{subproc:repair:l6}); 
if $\J.\texttt{cnt}[u]=0$ in addition (line~\ref{subproc:repair:l7}), 
then $u$ is (correctly) recognized as inconsistent, so it is inserted into $L^{\text{inc}}$ (line~\ref{subproc:repair:l8}).
This is also correct because $\J.\texttt{cnt}[u]$ was initialized to be $|N^{\text{out}}(u)|$, and $\J.\texttt{inc}[(u,v)]$ 
to be $\texttt{false}$, by $\texttt{init\_jumper}()$ (see SubProcedure~\ref{proc:jumper_init}, line~\ref{proc:jumper_init:l5} 
and line~\ref{proc:jumper_init:l7}). These operations are repeated until $L^{\text{inc}}\neq\emptyset$ or 
$L_{\text{\bf{w}}}=\emptyset$ (line~\ref{subproc:energy_jump:l3} of SubProcedure~\ref{subproc:energy_jumps}).
At that point, $\texttt{ei-jump}()$ returns \texttt{true} (line~\ref{subproc:energy_jump:l7}), 
and Algorithm~\ref{algo:solve_mpg} takes back control. Let $i'=\J.i$ at that point (line~\ref{algo:solve:l9}), 
observe $i'\in [W^-, W^+]$.So, notice that $\J.\texttt{cnt}$ and $\J.\texttt{inc}$ are kept coherent \wrt $f^{\text{c}}={\bf{0}}$, 
at least, until the $1$-th invocation of $\texttt{J-VI}()$ (line~\ref{algo:solve:l5} of Algorithm~\ref{algo:solve_mpg}); 
indeed $L_{\text{\bf{w}}}$ had been sorted in ascending order by $\texttt{init\_jumper}()$ 
at line~\ref{algo:solve:l5} of Algo.~\ref{algo:solve_mpg}. There, $\texttt{J-VI}()$ is finally invoked. 
The state of Algorithm~\ref{algo:solve_mpg} is now as follows, for some $i'\in [W^-, W^+]$ and $j=1$.

-- Let us prove (PC-1). The $L_f$ is empty and $f^{\text{c}}={\bf{0}}$ 
	(as initialized by $\texttt{init\_jumper}()$ at line~\ref{algo:solve:l5} of Algo.~\ref{algo:solve_mpg}), 
	so $f^{\text{c}}={\bf{0}}\preceq f^*_{w'_{i',1}}$. This proves (PC-1).  

-- Let us prove (w-PC-2). The $L^{\text{inc}}_{\text{nxt}}$ is empty (as initialized by 
	$\texttt{init\_jumper}()$ at line~\ref{algo:solve:l5} of Algo.~\ref{algo:solve_mpg}). 
	Also, any $v\in L^{\text{inc}}$ is inconsistent \wrt 
	to $f^{\text{c}}={\bf{0}}$ in $\Gamma_{i',j}$ (as already observed above). This proves (w-PC-2).  

-- Let us prove (w-PC-3). At this point, because of what was already mentioned above 
	concerning $\J.\texttt{cnt}$ and $\J.\texttt{inc}$, (w-PC-3) is also satisfied. 
	In particular, notice that (only for the Base Case) it holds $\J.\texttt{inc}[(u,v)]=\texttt{false}$ 
	if and only if $(u,v)\in E$ is compatible \wrt $f^\text{c}={\bf{0}}$ in $\Gamma_{i',j}$. This proves (w-PC-3). 

Therefore, (PC-1), (w-PC-2) and (w-PC-3) are all satisfied at the time of the 1-th invocation of $\texttt{J-VI}()$. 
	This proves the Base-Case of the induction.

\emph{Inductive Step.}
Let $k\in\N$, $k > 1$. Assume that (PC-1), (w-PC-2) and (w-PC-3) are all satisfied 
	at the time of the $k-1$-th invocation of $\texttt{J-VI}()$.
Assume that the $k-1$-th invocation of $\texttt{J-VI}()$ takes input $i=i_{k-1}$ and $j=j_{k-1}$, this may happen either 
 at line~\ref{algo:jvalue:l12} of Algorithm~\ref{algo:solve_mpg} or at line~\ref{subproc:ua-jumps:l3} of $\texttt{ua-jumps}()$ (SubProcedure~\ref{subproc:ua-jumps}).
By induction hypothesis, by Proposition~\ref{prop:saint_weak_coherency} and by Lemma~\ref{lem:jvalue_init_correct}, 
when the $k-1$-th halts, then $f^{\text{c}}$ is the least-SEPM of $\Gamma_{i_{k-1}, j_{k-1}}$, and $\J.\texttt{cnt}^{\text{c}}$, $\J.\texttt{inc}^{\text{c}}$ are both coherent 
\wrt $f^{\text{c}}$ in $\Gamma_{i_{k-1},j_{k-1}}$; 
moreover, by Proposition~\ref{prop:jvalue_init}, if $v\in L^{\text{inc}}$, 
	then $v$ is inconsistent \wrt $\J.f^{\text{c}}$ in $\Gamma_{i_{k-1}, j_{k-1}}$.
Now we prove that (PC-1), (w-PC-2) and (w-PC-3) are all satisfied just before the $k$-th invocation of $\texttt{J-VI}()$. 
The latter may also happen either at line~\ref{algo:jvalue:l12} of Algorithm~\ref{algo:solve_mpg} or at line~\ref{subproc:ua-jumps:l3} of $\texttt{ua-jumps}()$ (SubProcedure~\ref{subproc:ua-jumps}). 
	So, the proof is organized in four cases.  
\begin{itemize}
\item[Case 1.] Assume that both the $k-1$-th and the $k$-th invocation of $\texttt{J-VI()}$ happen at line~\ref{subproc:ua-jumps:l3} of $\texttt{ua-jumps}()$ (SubProcedure~\ref{subproc:ua-jumps}). 
\end{itemize}
			Then, the only operations that are carried out between 
			the end of the $k-1$-th and the beginning of the $k$-th invocation are the following:
			$i=i_{k-1}$ is incremented by one unit (at line~\ref{subproc:ua-jumps:l5} of $\texttt{ua-jumps}()$), so that $i_k=i_{k-1}+1$ and 
			$j_k=s-1$ (at line~\ref{subproc:ua-jumps:l3} of $\texttt{ua-jumps}()$);
			$\texttt{join\_ua-jump}(i_k, F, \J)$ is invoked (at line~\ref{subproc:ua-jumps:l6} of $\texttt{ua-jumps}()$) .			
				
			($\star$) The key point  is that $\texttt{join\_ua-jump}()$, 
			apart from copying $L_f$, $L_{\text{cnt}}$ and $L_{\text{inc-arc}}$ back to 
			$\J.f$, $\J.\texttt{cnt}$ and $\J.\texttt{inc}$ (respectively), 
			meanwhile emptying $L_f$, $L_{\text{cnt}}$, $L_{\text{inc-arc}}$, 
			it takes care of repairing the counters and \texttt{inc} 
			flags \wrt all those arcs $(u,v)\in E$ such that: 
			$w(u,v)=i_k=i_{k-1}+1$ and $\J.f[u]=\J.f[v]=0$ (if any);
			if, during such a repairing, any $\hat{u}\in V_0\setminus L^{\text{inc}}$ is recognized to be 
			inconsistent \wrt $f^{\text{c}}$ in $\Gamma_{i_k, s-1}$, 
			then $\hat{u}$ is (correctly) inserted into $L^{\text{inc}}$; 
			and this is the only way in which $\texttt{join\_ua-jump}()$ modifies $L^{\text{inc}}$. 
	
			With this in mind, we are now in position to carefully check all the preconditions.
	
			-- Let us prove (PC-1). As $\texttt{join\_ua-jump}()$ empties $L_f$, 
				then $L_f=\emptyset$ holds just before the $k$-th invocation of $\texttt{J-VI}()$. 
				Next, we argue that $f^{\text{c}}\preceq f^*_{w'_{i_k, s-1}}$. 
				When the $k-1$-th invocation of $\texttt{J-VI}()$ halts, 
				$f^{\text{c}}=f^*_{w'_{i_{k-1}, s-1}}$. 	
				Since $F_{s-1}=1$, 
				then it holds $w'_{i_{k-1}, s-1}= w_{i_{k-1}, s-1}$, 
				and $w'_{i_k, s-1}=w'_{i_{k-1}+1, s-1}=w_{i_{k-1}+1,s-1}=w_{i_k, s-1}$ 
				because $i_k=i_{k-1}+1$ in addition. 
				Since $i_k=i_{k-1}+1$, then $w_{i_k, s-1}=$. Therefore, we have:
				\begin{align*}
					f^{\text{c}} = f^*_{w'_{i_{k-1}, s-1}} = & f^*_{i_{k-1}, s-1} & 
									\text{[by $w'_{i_{k-1}, s-1}=w_{i_{k-1}, s-1}$]} \\ 
								\preceq & f^*_{i_{k-1}+1, s-1} & 
										\text{[by $w_{i_{k-1}+1, s-1} < w_{i_{k-1}, s-1}$]} \\ 
								= & f^*_{i_k, s-1} & \text{[by $i_k=i_{k-1}+1$]} \\ 
								= & f^*_{w'_{i_k, s-1}} & \text{[by $w'_{i_k, s-1}=w_{i_k, s-1}$]} 
				\end{align*}
				So, $f^{\text{c}}\preceq f^*_{w'_{i_k, s-1}}$. This proves (w-PC-1).
	
			-- Let us prove (w-PC-2). By Proposition~\ref{prop:jvalue_init}, all vertices that were already inside 
			$L^{\text{inc}}$ at the end of the $k-1$-th invocation of $\texttt{J-VI}()$, 
			they were all inconsistent \wrt $\J.f^{\text{c}}$ in $\Gamma_{i_{k-1}, s-1}$, 
			so they are still inconsistent \wrt $\J.f^{\text{c}}$ in $\Gamma_{i_k, s-1}$ 
			just before the $k$-th invocation of $\texttt{J-VI()}$, 
			because $i_k=i_{k-1}+1$ imply $w'_{i_k, s-1} < w'_{i_{k-1}, s-1}$. 
			Also notice $L^{\text{inc}}_{\text{nxt}}=\emptyset$. 
			These, with ($\star$), imply (w-PC-2). 
				
			-- Let us prove (w-PC-3).  
			When the $k-1$-th invocation of $\texttt{J-VI}()$ halts, 
			$\J.\texttt{cnt}^{\text{c}}$, $\J.\texttt{inc}^{\text{c}}$ are both coherent 
			\wrt $f^{\text{c}}$ in $\Gamma_{i_{k-1},j_{k-1}}=\Gamma_{i_{k-1},j_{s-1}}$. 
			Now, what can happen to them just before the $k$-th invocation 
			of $\texttt{J-VI}()$ on input $(i_k, s-1, F, \J)$, 
			considering the fact that $f^\texttt{c}$ stands still, $i_k=i_{k-1}+1$ and that ($\star$) holds ?
			To begin, since $\texttt{join\_ua-jump}()$
			copies $L_{\text{cnt}}$ and $L_{\text{inc-arc}}$ back to $\J.\texttt{cnt}$ and 
			$\J.\texttt{inc}$ (respectively), 
			then it is safe now to look at the coherency state of $\J.\texttt{cnt}$ and 
			$\J.\texttt{inc}$ \wrt $f^{\text{c}}$ in $\Gamma_{i_k, s-1}$.
			So, let $u\in V_0\setminus L^{\text{inc}}$ and $v\in N^{\text{out}}(u)$ (arbitraryly). 
			Since, when the $k-1$-th invocation of $\texttt{J-VI}()$ halted, 
			$\J.\texttt{cnt}^{\text{c}}$ was coherent 
			\wrt $f^{\text{c}}$ in $\Gamma_{i_{k-1},j_{s-1}}$, and since ($\star$) holds, then
			$\J.\texttt{cnt}[u] = \big\{ q \in N^{\text{out}}(u) \mid 
			\J.\texttt{inc}[(u,q)]=\texttt{false} \big\}$ 
			and $\J.\texttt{cnt}[u]>0$. This proves Item 1 of (w-PC-3).
			Concerning Item~2 of (w-PC-3), there are two possible cases. 
			\begin{itemize}
			\item	If $\J.\texttt{inc}[(u,v)]=\texttt{true}$, 
				then we argue that $(u,v)\in E$ is incompatible \wrt $f^{\text{c}}$ in $\Gamma_{i_k, s-1}$. 
					Indeed, either: (i) $\J.\texttt{inc}^{\text{c}}[(u,v)]=\texttt{true}$ was 
							already true at the end of the $k-1$-th invocation of $\texttt{J-VI}()$, 
							so that $(u,v)$ was incompatible 
							\wrt $f^{\text{c}}$ in $\Gamma_{i_{k-1}, s-1}$, 
							and therefore $(u,v)$ is now incompatible \wrt $f^{\text{c}}$ in 
							$\Gamma_{i_k, s-1}=\Gamma_{i_{k-1}+1, s-1}$ 
							(because $w'_{i_k, s-1} < w'_{i_{k-1}, s-1}$);
						or (ii) at the end of the $k-1$-th invocation of $\texttt{J-VI}()$, 
							it was $\J.\texttt{inc}^{\text{c}}[(u,v)]=\texttt{false}$,  
							and $\texttt{join\_ua-jump}(i_k, F, \J)$ repaired it by setting 
							$\J.\texttt{inc}[(u,v)]=\texttt{true}$, 
							but this (correctly) happens if and only if $w(u,v)=i_k=i_{k-1}+1$ 
							and $\J.f[u]=\J.f[v]=0$, so that $(u,v)$ is now incompatible 
							\wrt $f^{\text{c}}$ in $\Gamma_{i_k, s-1}$. In both cases, the claim holds. 
			\item	Else, it holds $\J.\texttt{inc}[(u,v)]=\texttt{false}$, 
				then we argue that either $(u,v)$ is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i_k, s-1}$ or it holds that $v\in L^{\text{inc}}$. 
				Indeed, assume that $\J.\texttt{inc}[(u,v)]=\texttt{false}$ and 
				that $(u,v)$ is incompatible \wrt $f^{\text{c}}$ in $\Gamma_{i_k, s-1}$.
				Since $\J.\texttt{inc}[(u,v)]=\texttt{false}$, then it was as such even at 
				the halting time of the $k-1$-th invocation of $\texttt{J-VI}()$, 
				before the last invocation of $\texttt{join\_ua-jump}()$, because the latter 
				can (possibly) switch the state of $\J.\texttt{inc}$ only from \texttt{false} to \texttt{true}.
				Therefore, $(u,v)$ was compatible \wrt $f^{\text{c}}$ in $\Gamma_{i_{k-1}, s-1}$. 
				But $(u,v)$ is now incompatible \wrt $f^{\text{c}}$ in $\Gamma_{i_k, s-1}$, 
				still, $\J.\texttt{inc}[(u,v)]=\texttt{false}$; this means that the last invocation of $\texttt{join\_ua-jump}()$ has not recognized 
				$(u,v)$ as incompatible. Therefore, it must be that either $\J.f[u]>0$ or $\J.f[v]>0$. 
				At the halting time of the $k-1$-th invocation of $\texttt{J-VI}()$, 
				it holds that $L^{\text{inc}}=\{q\in V\mid 0<f^{\texttt{c}}(q)\neq\top\}$ 
				by Proposition~\ref{prop:jvalue_init}. Notice that, since the $k-1$-th and the $k$-th invocation 
				of $\texttt{J-VI}()$ are both executed at line~\ref{subproc:ua-jumps:l3} of 
				$\texttt{ua-jumps}()$ (SubProcedure~\ref{subproc:ua-jumps}), 
				then $L_\top=\emptyset$ line~\ref{subproc:ua-jumps:l4} of $\texttt{ua-jumps}()$, 
				so that $u\not\in L_\top$, \ie $f^{\text{c}}(u)\neq\top$.
				Since $u\in V_0\setminus (L^{\text{inc}}\cup L_\top)$, then, 
				it must be $\J.f[u]=0$, therefore, $\J.f[v]>0$, so that $v\in L^{\text{inc}}$. 
			\end{itemize}
			These prove Item~2 of (w-PC-3). So, (w-PC-3) holds.
\begin{itemize}					
\item[Case 2.] Assume that the $k-1$-th invocation of $\texttt{J-VI()}$ happens at line~\ref{subproc:ua-jumps:l3} of $\texttt{ua-jumps}()$, 
		and that the $k$-th happens at line~\ref{algo:solve:l12} of Algorithm~\ref{algo:solve_mpg}.  
\end{itemize}
		When the $k-1$-th one halts, it must be that $L_\top\neq\emptyset$ 
		(otherwise we would had not came out of the \texttt{repeat-until} loop at line~7 of $\texttt{ua-jumps}()$,   
		and we would had not reached line~\ref{algo:solve:l12} of Algorithm~\ref{algo:solve_mpg}). 
		So, the only operations that are carried out between the end of the $k-1$-th and the beginning 
		of the $k$-th invocation of $\texttt{J-VI}()$ are just \emph{backtracking} operations: 
		$\texttt{stop\_ua-jumps}(\J)$ is invoked at line~\ref{subproc:ua-jumps:l8} of $\texttt{ua-jumps}()$, 
		and $j\leftarrow 1$ is assigned (line~\ref{algo:solve:l11} of Algorithm~\ref{algo:solve_mpg}).  
		What $\texttt{stop\_ua-jumps}(\J)$ does, is just restoring the state of $L^{\text{inc}}$ 
		as it was just before the $k-1$-th invocation of $\texttt{J-VI}()$; 
		and to clear the state of $L^{\text{inc}}_{\text{cpy}}$, 
		$L_\top$, $L_{\text{cnt}}$, $L_f$, $L_{\text{inc-arc}}$ (line~\ref{subproc:unitary_stop:l2}), 
		thus restoring the state of $\J.\texttt{cnt}^{\text{c}}$ and that of 
		$\J.\texttt{inc}^{\text{c}}$ as it was just before the $k-1$-th invocation of $\texttt{J-VI}()$; finally, 
		to set $\J.\texttt{ua-jump\_mode}\leftarrow\texttt{false}$ (line~\ref{subproc:unitary_stop:l3}).
		So, just before the $k$-th invocation of $\texttt{J-VI}()$ at line~\ref{algo:solve:l12} of Algorithm~\ref{algo:solve_mpg}, 
		the state of $\J$ is restored so to be (almost) the same as it was just before the $k-1$-th invocation of $\texttt{J-VI}()$ 
		(the only difference being $\J.\texttt{ua-jump\_mode}$, $L^{\text{inc}}_{\text{cpy}}$, 
		but they are not essential \wrt whether the preconditions hold or not). 
		Therefore, since (PC-1), (w-PC-2) and (w-PC-3) hold just before the $k-1$-th invocation of $\texttt{J-VI}()$, 
		they must hold now just before the $k$-th invocation as well (because the backtracking step restored the state).
\begin{itemize}
\item[Case 3.] Assume that the $k-1$-th invocation of $\texttt{J-VI()}$ happens at line~\ref{algo:solve:l12} 
		of Algorithm~\ref{algo:solve_mpg}, and that the $k$-th happens at line~\ref{subproc:ua-jumps:l3} of $\texttt{ua-jumps}()$.
\end{itemize}
		The operations that are carried out between the end of the $k-1$-th and the beginning 
		of the $k$-th invocation are the following: $\texttt{set\_vars}()$ is invoked (line~\ref{algo:solve:l13}), 
		but only this changes the state of $\W_0,\W_1,\nu,\sigma_0^*$, and $L_\top$ (emptying it); next, 
		$\texttt{scl\_back\_}$f$(j,F,\J)$ is invoked (line~\ref{algo:solve:l14}), 
		and this (correctly) scales and copies back the (integral) energy-levels of $L_f$ to those of $\J.f$ (which are rational);  
	   	next, $j\leftarrow j+1$ is assigned (line~\ref{algo:solve:l15}); then $\texttt{ei-jump}(i,j,\J)$ is executed (line~\ref{algo:solve:l8}). Let $i_s\triangleq i$ at that point. 
		Since the $k$-th happens at line~\ref{subproc:ua-jumps:l3} of $\texttt{ua-jumps}()$, then $\texttt{ei-jump}()$ must have returned \texttt{true}, 
		so that $i\leftarrow \J.i$ is assigned (line~\ref{algo:solve:l10} of Algorithm~\ref{algo:solve_mpg}). 
		Let $i_t\triangleq \J.i$ at that point, \ie at line~\ref{algo:solve:l10}. By Lemma~\ref{lem:ei-jump_state}, $i_t > i_s$. 
		Next, $\texttt{init\_ua\_jumps}(\J)$ is invoked (line~\ref{subproc:ua-jumps:l1} of $\texttt{ua-jumps}()$) 
		(which backup copies $L^{\text{inc}}$ to $L^{\text{inc}}_{\text{cpy}}$, 
		and assigns the flag $\J.\texttt{ua-jump\_mode}\leftarrow\texttt{true}$).  
	
	($\star\star$) Now, he key point is that $\texttt{ei-jump}(i_s,j,\J)$ (line~\ref{algo:solve:l8})
		takes care of repairing the counters and \texttt{inc} flags \wrt all those arcs $(u,v)\in E$ such that: 
		$i_s+1\leq w(u,v)\leq i_t$ and $\J.f[u]=\J.f[v]=0$ (if any);
		if, during such a repairing, any $\hat{u}\in V_0\setminus L^{\text{inc}}$ is 
		recognized to be inconsistent \wrt $f^{\text{c}}$ in $\Gamma_{i', 1}$, some $i_s+1\leq i'\leq i_t$, 
		then $\hat{u}$ is (correctly) inserted into $L^{\text{inc}}$; 
		and this is the only way in which $\texttt{ei-jump}(i_s,j,\J)$ modifies $L^{\text{inc}}$. 
		Notice that any such $\hat{u}$ is also inconsistent \wrt $f^{\text{c}}$ 
		in $\Gamma_{\bar{i}, \bar{j}}$ 
for any $(\bar{i}, \bar{j})> (i', 1)$.
	
		With this in mind, we are now in position to carefully check all the preconditions.
		
		-- Let us prove (PC-1). 
		As $\texttt{stop\_ua-jumps}()$ empties $L_f$, 
		$L_f=\emptyset$ holds just before the $k$-th invocation of $\texttt{J-VI}()$.
		Next, when the $k-1$-th invocation of $\texttt{J-VI}()$ halts, 
		then $f^{\text{c}}=f^*_{w'_{i_{k-1}, j_{k-1}}}=f^*_{w'_{i_s, j_{k-1}}}$.
		Since the subprocedure $\texttt{scl\_back\_}$f$(j_{k-1},F,\J)$ is invoked (line~\ref{algo:solve:l14}) soon after, 
		then $f^{\text{c}}$ is scaled back by setting $\J.f=f^*_{i_s, j_{k-1}}$.
		Recall that the $k$-th invocation of $\texttt{J-VI}()$ is invoked on input $(i_t, s-1)$. 
		Since $(i_s, j_{k-1}) < (i_t, s-1)$, by Lemma~\ref{lem:monotone_energy}  
		it holds that $f^*_{i_s, j_{k-1}}\preceq f^*_{i_t, s-1}$. Since $F_{s-1}=1$, then $w_{i_t, s-1}=w'_{i_t, s-1}$, 
		therefore, $f^*_{i_t, s-1}= f^*_{w'_{i_t, s-1}}$; 
		also, $D_{s-1} f^*_{i_s, j_{k-1}}= f^*_{i_s, j_{k-1}}$, as the denominator of $F_{s-1}$ is $D_{s-1}=1$. 
		Thus $D_{s-1} f^*_{i_s, j_{k-1}} \preceq f^*_{w'_{i_t, s-1}}$. 
			Since $f^*_{w'_{i_t, s-1}}(v)\in\Z$ for every $v\in V$, 
			then $\lceil D_{s-1} f^*_{i_s, j_{k-1}} \rceil \preceq f^*_{w'_{i_t, s-1}}$. 
		At the time of the $k$-th invocation of $\texttt{J-VI}()$, 
		it holds that $f^{\text{c}}=\lceil D_{s-1} f^*_{i_s, j_{k-1}}\rceil$. 
		So, $f^{\text{c}}\preceq f^*_{w'_{i_t, s-1}}$.
		This proves (PC-1).

		-- Let us prove (w-PC-2). By Proposition~\ref{prop:jvalue_init}, 
		all vertices that were already inside $L^{\text{inc}}$ at the end of the $k-1$-th invocation of $\texttt{J-VI}()$, 
		they were all inconsistent \wrt $\J.f^{\text{c}}$ in $\Gamma_{i_s, j_{k-1}}$, 
		so they are still inconsistent \wrt $\J.f^{\text{c}}$ in $\Gamma_{i_t, s-1}$ 
		just before the $k$-th invocation of $\texttt{J-VI()}$, because $(i_s, j_{k-1}) < (i_t, s-1)$. 
		Also, $L^{\text{inc}}_{\text{nxt}}=\emptyset$ at the end of the $k-1$-th invocation of $\texttt{J-VI}()$. 
		These facts, plus ($\star\star$), imply (w-PC-2). 
	
		-- Thee proof of (w-PC-3) proceeds as in Case~1. The only remarkable difference is that now ($\star\star$) holds, 
			instad of ($\star$); so, the repairing of $\J.\texttt{cnt}$ and $\J.\texttt{inc}$ may happen, 
			within $\texttt{ei-jump}()$ (line~\ref{algo:solve:l8} of Algo.~\ref{algo:solve_mpg}) 
			for more than one weight value $i'$ such that $i_s+1\leq i'\leq i_t$, 
			until either $L^{\text{inc}}\neq\emptyset$ or $L_{\text{\bf{w}}}=\emptyset$ 
			(see line~\ref{subproc:energy_jump:l3} of SubProcedure~\ref{subproc:energy_jumps}). 
			Apart from that the proof of (w-PC-3) is the same.
\begin{itemize}
\item[Case 4.] Assume that both the $k-1$-th and the $k$-th invocation of $\texttt{J-VI()}$ happen at line~\ref{algo:solve:l12} of Algorithm~\ref{algo:solve_mpg}. 
\end{itemize}
		The operations that are carried out between the end of the $k-1$-th and the beginning of the $k$-th invocation 
		are the following: $\texttt{set\_vars}()$ is invoked (line~\ref{algo:solve:l13}), 
		this may (possibly )change the state of $\W_0,\W_1,\nu,\sigma_0^*$, and that of $L_\top$ (emptying it); next, 
		$\texttt{scl\_back\_}$f$(j,F,\J)$ is invoked (line~\ref{algo:solve:l14}), 
		this scales and copies back the (integral) energy-levels of $L_f$ to those of $\J.f$ (rational); 
		next, $j\leftarrow j+1$ is incremented (line~\ref{algo:solve:l15}). 
		So, $i_k=i_{k-1}$ and $j_k=j_{k-1}+1$. Then $\texttt{ei-jump}(i,j,\J)$ is executed (line~\ref{algo:solve:l8}).  
		Since the $k$-th invocation of $\texttt{J-VI}()$ also happens at line~\ref{algo:solve:l12} of Algorithm~\ref{algo:solve_mpg}, 
		then $\texttt{ei-jump}()$ must had returned \texttt{false}. So, when $\texttt{ei-jump}()$ is invoked, 
		it must had been that $L^{\text{inc}}\neq\emptyset$ and that $j<s$. Also 
		notice that $\J.\texttt{cnt}^{\text{c}}$ and $\J.\texttt{inc}^{\text{c}}$ are 
		not modified throughout the above mentioned operations. 
		With this in mind, at this point, it is not difficult to check 
		that (PC-1), (w-PC-2) and (w-PC-3) are all satisfied just before the $k$-th invocation of $\texttt{J-VI}()$. 
		Indeed, almost all relevant arguments have already appeared in the proof of the previous cases.
		the only relevant point that deserves to be mentioned is that, 
		since $i_k=i_{k-1}$ (and $j_k=j_{k-1}+1<s$) holds, 
		there is no $(u,v)\in E$ such that: $(u,v)$ was compatible \wrt $f^{\text{c}}$ in $\Gamma_{i_{k-1}, j_{k-1}}$, 
		$(u,v)$ is now incompatible \wrt $f^{\text{c}}$ in $\Gamma_{i_{k}, j_{k}}=\Gamma_{i_{k-1}, j_{k-1}+1}$  
		and $\J.f[u]=\J.f[v]=0$ holds at the same time. So, the fact that the $\texttt{ei-jump}()$ repairs 
		no counter nor \texttt{inc} flag is correct in this case. 

This proves that (PC-1), (w-PC-2) and (w-PC-3) are all satisfied just 
	before the $k$-th invocation of $\texttt{J-VI}()$, anyway.
\end{proof}

\subsection{Proof of Proposition~\ref{prop:ei-jump_correctness}}\label{subsect:ei-jump_correctness}

Notice, under the hypotheses of 
Proposition~\ref{prop:ei-jump_correctness}, $f^{\text{c}}$ stands still during $\texttt{ei-jump}()$, 
$f^{\text{c}:\iota}=f^{\text{c}:\iota'}=f^{\text{c}:\iota''}=f^{\text{c}:h}$. 
So, in the proof below, we can refer only to $f^{\text{c}}$.
 
\begin{itemize}
\item[\emph{Proof Item (1)}] 
\end{itemize}
-- Assume it is the first time that Algorithm~\ref{algo:solve_mpg} invokes 
$\texttt{ei-jump}()$ (SubProcedure~\ref{subproc:energy_jumps}) (line~\ref{algo:solve:l8}).
So, $i=W^-$ and $j=1$ (line~\ref{algo:solve:l6} of Algorithm~\ref{algo:solve_mpg}),
and $\forall (v\in V) f^{\text{c}}(v)=0$ (as initialized by $\texttt{init\_jumper}()$, 
	line~\ref{proc:jumper_init:l4} of SubProcedure~\ref{proc:jumper_init}) (1.a). 
Next, $\text{Inc}(f^{\text{c}}, i, j-1)=\text{Inc}(f^{\text{c}}, W^-, 0)=\emptyset$, 
	because $\forall (e\in E) w'_{W^-,0}(e)\geq 0$ (1.b).
Moreover, $\forall (u\in V_0) \J.\texttt{cnt}^\iota[u]=|N^{\text{out}}(u)|$, and 
$\forall (v\in N^{\text{out}}(u))\J.\texttt{inc}^\iota[(u,v)]=\texttt{F}$ (see $\texttt{init\_jumper}()$,  
	lines~\ref{proc:jumper_init:l5}-\ref{proc:jumper_init:l7} of SubProcedure~\ref{proc:jumper_init}).
So, when $\texttt{ei-jump}(W^-,1,s,\J)$ is invoked, 
$\J.\texttt{cnt}^\iota$ and $\J.\texttt{inc}^\iota$ are coherent 
\wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}=\Gamma_{W^-,0}$ (1.c).

-- Consider any other invocation of 
$\texttt{ei-jump}()$ (SubProcedure~\ref{subproc:energy_jumps}) (line~\ref{algo:solve:l8}). 
Before that, $\texttt{J-VI}(i,j-1,F,\J,\Gamma)$ (SubProcedure~\ref{algo:j-value-iteration}) 
must had been invoked (line~\ref{algo:solve:l12}), say at step $\iota_0$. 
Assume $\texttt{J-VI}(i,j-1,F,\J,\Gamma)$ (line~\ref{algo:solve:l12}) halts at step $\iota_1$. 
Notice, $\J.\texttt{cnt}^{\iota}=\J.\texttt{cnt}^{\iota_1}$, 
$\J.\texttt{inc}^{\iota}=\J.\texttt{inc}^{\iota_1}$, 
as lines~\ref{algo:solve:l13}-\ref{algo:solve:l15} (Algorithm~\ref{algo:solve_mpg}) don't alter them; 
so, we refer only $\iota$. 
By Proposition~\ref{prop:saint_weak_coherency_holds}, 
all of (PC-1), (w-PC-2), (w-PC-3) hold at $\iota_0$. 
By Proposition~\ref{prop:saint_weak_coherency}, (w-PC-2), (w-PC-3) can safely replace (PC-2), (PC-3).
By Item~1 of Proposition~\ref{prop:saint_weak_coherency}, 
$f^{\text{c}}=f^*_{w'_{i,j-1}}$.
By Item~3 of Proposition~\ref{prop:saint_weak_coherency}, 
${L^{\text{inc}}}^{\iota} = \{ v\in V \mid 0<f^{\text{c}}(v) \neq \top \}$; 
since ${L^{\text{inc}}}^{\iota}=\emptyset$, then, 
$\forall (v\in V)$ either $f^{\text{c}}(v)=0$ or $f^{\text{c}}(v)=\top$. (1.a). 
By Item~1 of Proposition~\ref{prop:saint_weak_coherency}, 
$f^{\text{c}}$ is the least-SEPM of $\Gamma_{i,j-1}$, therefore, 
\emph{no} $v\in V$ is inconsistent \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$ (1.b).
By Item~2 of Proposition~\ref{prop:saint_weak_coherency}, $\J.\texttt{cnt}^{\iota}$, 
$\J.\texttt{inc}^{\iota}$ are coherent \wrt $f^{\text{c}}$ in 
$\Gamma_{i,j-1}$ (1.c).

This concludes the proof of (1). $\square$

\begin{itemize}
\item[\emph{Proof of Item (2)}] Let $u\in V_0$, $v\in N^{\text{out}}(u)$, 
	and let $(i',j')$ be fixed such that $(i,j-1) < (i',j')\leq (i^h,1)$. 
\end{itemize}

By (1.a), either $f^{\text{c}}(u)=\top$ or $f^{\text{c}}(u)=0$, and either $f^{\text{c}}(v)=\top$ or $f^{\text{c}}(v)=0$. 
\begin{itemize}
\item If $f^{\text{c}}(u)=\top$, then  
	$(u,v)\in E$ is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$. 
	So, $\J.\texttt{inc}^{\iota}[(u,v)]=\texttt{F}$ holds by (1.c).
	Since $f^{\text{c}}(u)=\top$, $\texttt{ei-jump}()$ can't modify $\J.\texttt{inc}[(u,v)]$, 
	see line~\ref{subproc:repair:l2} of $\texttt{repair}()$ (SubProcedure~\ref{subproc:energy_jumps}).
	As $f^{\text{c}}(u)$ and $\J.\texttt{inc}[(u,v)]$ stand still, 
	then $\J.\texttt{inc}^{\iota''}[(u,v)]=\texttt{F}$ 
	is coherent \wrt $f^{\text{c}}(u)=\top$ in $\Gamma_{i',j'}$.
	
\item If $f^{\text{c}}(u)=0$ and $f^{\text{c}}(v)=\top$, 
then $(u,v)\in E$ is incompatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$. 
So, $\J.\texttt{inc}^{\iota}[(u,v)]=\texttt{T}$ holds by (1.c);
then, it holds for the whole execution of $\texttt{ei-jump}()$ as well, 
because $\texttt{ei-jump}()$ (SubProcedure~\ref{subproc:energy_jumps})
never switches $\J.\texttt{inc}$ from \texttt{T} to \texttt{F}.  
Again, as $f^{\text{c}}(u)$ and $\J.\texttt{inc}[(u,v)]$ stand still, 
		$\J.\texttt{inc}^{\iota''}[(u,v)]=\texttt{T}$ 
is coherent \wrt $f^{\text{c}}(u)=0$ in $\Gamma_{i',j'}$.

\item Assume $f^{\text{c}}(u)=0$ and $f^{\text{c}}(v)=0$. 

Recall, $\J.\texttt{inc}[(u,v)]$ is coherent \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$ by (1.c). Then, 
\begin{itemize}
\item If $\J.\texttt{inc}^{\iota}[(u,v)]=\texttt{T}$, 
then $(u,v)$ is incompatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$.
Thus, since $f^{\text{c}}(u)=f^{\text{c}}(v)=0$ and $j'\in [1,s-1]$, 
then $w(u,v)\leq i$. Since $i\leq i'$, then $w(u,v)\leq i'$; 
this means that $(u,v)$ is still incompatible \wrt $f^{\text{c}}$ in $\Gamma_{i',j'}$.
Meanwhile, $\J.\texttt{inc}[(u,v)]=\texttt{T}$ stands still  
(because $\texttt{ei-jump}()$ never switches the value 
of $\J.\texttt{inc}[(u,v)]$ from \texttt{T} to \texttt{F}), 
so $\J.\texttt{inc}[(u,v)]=\texttt{T}$.

\item If $\J.\texttt{inc}^{\iota}[(u,v)]=\texttt{F}$, 
then $(u,v)$ is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$ by (1.c). So,  
\begin{itemize} \item If $(u,v)$ is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i',j'}$, 
then $w(u,v)>i'$; because $f^{\text{c}}(u)=f^{\text{c}}(v)=0$ and $j'\in [1,s-1]$.
Consider what happens in $\texttt{ei-jump}()$ at $\iota'$. 
Since $L_{\text{\bf{w}}}$ is sorted in increasing order, 
and since $w(u,v)>i'$, then the entry $(w(u,v), L_{\alpha})$ 
is still inside $L_{\text{\bf{w}}}$ at $\iota'$.  
Therefore, neither the subsequent invocation of $\texttt{repair}()$ 
(line~\ref{subproc:energy_jump:l6} of SubProcedure~\ref{subproc:energy_jumps}), 
nor the previous invocations of $\texttt{repair}()$ before $\iota'$, 
can switch the state of $\J.\texttt{inc}([u,v])$ from $\texttt{F}$ to $\texttt{T}$, 
just because $(u,v)\in L_\alpha$ is still kept inside $L_{\text{\bf{w}}}$; so, 
$\J.\texttt{inc}([u,v])=\texttt{F}$ stands still. 

\item If $(u,v)\in E$ is incompatible \wrt $f^{\text{c}}$ in $\Gamma_{i',j'}$, then $w(u,v)\leq i'$ 
(because $f^{\text{c}}(u)=f^{\text{c}}(v)=0$ and $j'\in [1,s-1]$). 
Since $w(u,v)\leq i'$, there is some step $\iota\leq \hat{\iota} <\iota'$  
at which the entry $(w(u,v), L_{\alpha})$ is popped from $L_{\text{\bf{w}}}$.  
Soon after $\hat{\iota}$, the subsequent invocation of 
$\texttt{repair}()$ (line~\ref{subproc:energy_jump:l6} of 
SubProcedure~\ref{subproc:energy_jumps}) alters the state 
of $\J.\texttt{inc}^{\hat\iota}[(u,v)]$ from $\texttt{F}$ to $\texttt{T}$, 
and it decrements $\J.\texttt{cnt}^{\hat\iota}[(u,v)]$ by one unit. So, $\J.\texttt{inc}$ is 
\emph{repaired} to be coherent \wrt $f^{\text{c}}$ in $\Gamma_{w(u,v),j'}$.
Now, $\J.i$ can only increase during the execution of $\texttt{ei-jump}()$, 
because $L_{\text{\bf{w}}}$ was sorted in increasing order.
So, from that point on, $(u,v)$ remains incompatible \wrt $f^{\text{c}}$ 
in $\Gamma_{\J.i,j'}$ for every $w(u,v) \leq \J.i\leq i'$. 
On the other hand, $\J.\texttt{inc}^{\hat\iota}[(u,v)]=\texttt{T}$ stands still, 
as $\texttt{ei-jump}()$ (SubProcedure~\ref{subproc:energy_jumps}) 
never switches it from \texttt{T} to \texttt{F}.    
\end{itemize}
In either case, $\J.\texttt{inc}^{\iota''}[(u,v)]$ is coherent 
\wrt $f^{\text{c}:\iota''}$ in $\Gamma_{i',j'}$.
\end{itemize}
So, $\J.\texttt{cnt}^{\iota''}$ is also coherent \wrt $f^{\text{c}:\iota''}$ in $\Gamma_{i',j'}$: 
indeed, it was coherent \wrt $f^{\text{c}:\iota}$ in $\Gamma_{i,j-1}$ by (1.c); 
then $\J.\texttt{cnt}$ was decremented by one unit (line~\ref{subproc:repair:l5} of $\texttt{repair}()$) 
each time that $\J.\texttt{inc}$ got 
repaired (line~\ref{subproc:repair:l6} of $\texttt{repair}()$), as described above; 
therefore, the coherency of $\J.\texttt{cnt}$ follows by that of $\J.\texttt{inc}$.
\end{itemize}
This proves (2). $\square$

\begin{itemize}
\item[\emph{Proof of Item (3)}]
\end{itemize}
Let $u\in V$ be any vertex. We show that $u\in V$ is consistent 
\wrt $f^{\text{c}}$ in $\Gamma_{i',j'}$ for every 
$i'\in [W^-,W^+]$ and $j'\in [1,s-1]$ such that $(i,j-1)<(i',j')<(i^h,1)$ (if any). 

By (1.a), either $f^{\text{c}}(u)=0$ or $f^{\text{c}}(u)=\top$. 
If $f^{\text{c}}(u)=\top$, the claim holds trivially. 

So, assume $f^{\text{c}}(u)=0$. By (1.b), $u$ is consistent \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$. 
Then, 
\begin{itemize} \item[Case $u\in V_0$.]  
By (1.c), $\J.\texttt{cnt}^{\iota}[u]$ is coherent \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$. 
Thus, $\J.\texttt{cnt}^{\iota}[u]>0$. Now, since $(i',j')<(i^h,1)$, 
then ${L^{\text{inc}}}^{\iota''}=\emptyset$. Therefore, 
$\J.\texttt{cnt}^{\iota''}[u]>0$ (otherwise $u$ would have been inserted 
into $L^{\text{inc}}$ within $\iota''$, see 
lines~\ref{subproc:repair:l7}-\ref{subproc:repair:l8} of $\texttt{repair}()$). 
By (2), $\J.\texttt{cnt}^{\iota''}[u]$ is coherent \wrt $f^{\text{c}}$ in $\Gamma_{i',j'}$.
Since $\J.\texttt{cnt}^{\iota''}[u]>0$ and $\J.\texttt{cnt}[u]^{\iota''}$ 
is coherent, then $u$ is consistent \wrt $f^\text{c}$ in $\Gamma_{i',j'}$. 

\item[Case $u\in V_1$.] Since $(i',j')<(i^h,i)$, then ${L^{\text{inc}}}^{\iota''}=\emptyset$. 
Let $v\in N^{\text{out}}(u)$. By (1.a) either $f^{\text{c}}(v)=0$ or $f^{\text{c}}(v)=\top$. 
Since $f^{\text{c}}(u)=0$, $u\in V_1$, 
and $u$ is consistent \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$ by (1.b), 
then $f^{\text{c}}(v)=0$.

Now, we claim that $w(u,v)>i'$.

Assume, for the sake of contradiction, that $w(u,v)\leq i'$. 
Recall, within $\iota'$, the entry $(i', L_{\alpha_1})$ is popped from 
$L_{\text{\bf{w}}}$ at line~\ref{subproc:energy_jump:l3} 
of $\texttt{ei-jump}()$ (SubProcedure~\ref{subproc:energy_jumps}).
Since $w(u,v)\leq i'$ and $L_{\text{\bf{w}}}$ was sorted in increasing order, 
the entry $(w(u,v), L_{\alpha_2})$ must have been consumed before $\iota'$.
The only lines of Algorithm~\ref{algo:solve_mpg} in which 
$(w(u,v), L_{\alpha_2})$ can have been consumed are: 
line~\ref{subproc:energy_jump:l3} or line~\ref{subproc:energy_jump:l12} 
of $\texttt{ei-jump}()$ (SubProcedure~\ref{subproc:energy_jumps}), 
or line~\ref{subproc:unitary_join:l7} of $\texttt{join\_ua-jump}()$ (SubProcedure~\ref{subproc:ua-jumps}).
Notice that, soon after any of these lines: 
$\texttt{repair}()$ takes care of inserting $u$ into $L^{\text{inc}}$ 
(because $u\in L_{\alpha_2}\cap V_1$ and $f^{\text{c}}(u)=f^{\text{c}}(v)=0$);
and, soon after that, say at step $\bar\iota$, it holds that $i^{\bar\iota}\geq w(u,v)$.
Still, ${L^{\text{inc}}}^{\iota''}=\emptyset$; 
so, $u$ must have been removed from $L^{\text{inc}}$, 
after $\bar\iota$ and before $\iota$.
Notice that $u$ can have been removed from $L^{\text{inc}}$ 
only at some execution of line~\ref{algo:jvalue:l2} 
of $\texttt{J-VI()}$ (SubProcedure~\ref{algo:j-value-iteration}), 
say at step $\bar{\iota}'$ for some $\bar\iota<\bar{\iota}'<\iota$.
Also, it is easy to check that $i^{\bar{\iota}'}\geq i^{\bar\iota}\geq w(u,v)$; 
thus, when $u\in V_1$ is removed from $L^{\text{inc}}$, 
$(u,v)$ is incompatible with $f^{\text{c}:\bar{\iota}'}$ 
in $\Gamma_{i^{\bar{\iota}'}, j^{\bar{\iota}'}}$ (because 
$f^{\text{c}:\bar{\iota}'}(u)=f^{\text{c}:\bar{\iota}'}(v)=0$, $i^{\bar{\iota}'}\geq w(u,v)$ 
and $j^{\bar{\iota}'}\geq 1$).
Since $u\in V_1$, then $u$ is also inconsistent.
Soon after in the $\texttt{J-VI}()$, at line~\ref{algo:jvalue:l3}, 
it is applied $\delta(f^{\text{c}:\bar{\iota}'}, u)$; 
since $u$ is really inconsistent, then the energy-level of $u$ must increase.
At that point, the energy-level of $u$ can't be zero. 
This would contradict the fact that $f^{\text{c}:\iota}(u)=0$;
but there is still one subtle detail in our argument, which it is worth clarifying. 
Even if the energy-level of $u$ increases thanks to $\delta(f^{\text{c}:\bar{\iota}'}, u)$ as mentioned above, 
it may well be the case that the energy-level of $u$ is restored back to be zero, soon after the end of the   
same $\texttt{J-VI}()$ which raised $f^{\text{c}:\bar{\iota}'}(u)$: this may happen at 
line~\ref{subproc:unitary_stop:l2} of $\texttt{stop\_ua-jumps}()$ (SubProcedure~\ref{subproc:ua-jumps}), 
when some UA-Jump's backtracking step occurs. 
Notice that, in this case, the $\texttt{J-VI}()$ which raised $f^{\text{c}:\bar{\iota}'}(u)$ was invoked at 
line~\ref{subproc:ua-jumps:l3} of $\texttt{ua-jumps}()$ (SubProcedure~\ref{subproc:ua-jumps}). 
Still, even in this case, the state of $L^{\text{inc}}$ is restored as well,  
at line~\ref{subproc:unitary_stop:l1} of $\texttt{stop\_ua-jumps}()$ (SubProcedure~\ref{subproc:ua-jumps}). 
Therefore, soon after that $\texttt{stop\_ua-jumps}()$ (SubProcedure~\ref{subproc:ua-jumps}) halts, 
$u$ is still inside $L^{\text{inc}}$, 
the value of $i$ stands still (\ie $i^{\bar{\iota}'}$), 
and Algorithm~\ref{algo:solve_mpg} has to execute 
yet another $\texttt{J-VI}()$; this time at line~\ref{algo:solve:l12}.
This one really has to increase the energy-level of $u$, 
which is therefore confirmed to be greater than zero at $\iota$. 
This also confirms, even in the case of UA-Jump's backtracking, 
that assuming $w(u,v)\leq i'$ leads to a contradicition.
Therefore, $w(u,v)>i'$. 

Since $\forall(v\in N^{\text{out}}(u))$$(w(u,v)>i'$ and $f^{\texttt{c}}(u)=f^{\texttt{c}}(v)=0)$, 
then $u$ is consistent \wrt $f^{\text{c}}$ in $\Gamma_{i',j'}$.
\end{itemize}
In either case, $u$ is consistent \wrt $f^{\text{c}}$ in $\Gamma_{i',j'}$. This proves (3). $\square$

\begin{itemize}
\item[\emph{Proof of Item (4)}]
\end{itemize}
Thanks to line~\ref{subproc:energy_jump:l2} of \texttt{ei-jump}() (SubProcedure~\ref{subproc:energy_jumps}), 
when the \texttt{while} loop at lines~\ref{subproc:energy_jump:l2}-\ref{subproc:energy_jump:l5} exits, 
then either ${L^{\text{inc}}}^{h}\neq\emptyset$ or both 
${L^{\text{inc}}}^h=\emptyset$ and $L^h_{\text{\bf{w}}}=\emptyset$.
Now, we want to prove that ${L^{\text{inc}}}^h=\text{Inc}(f^{\text{c}:h}, i^h, 1)$.
\begin{itemize}
\item ${L^{\text{inc}}}^h\subseteq \text{Inc}(f^{\text{c}:h}, i^h, 1)$:
\end{itemize}
Assume $u\in {L^{\text{inc}}}^h$. Then, either: 

-- $u\in V_0$ and $\J.\texttt{cnt}^{h}[u]=0$ 
	(see line~\ref{subproc:repair:l7} of $\texttt{repair}()$, 
	SubProcedure~\ref{subproc:energy_jumps}).

	In this case, by (2), $\J.\texttt{cnt}^{h}[u]$ is coherent \wrt $f^{\text{c}}$ in $\Gamma_{i^h,1}$;
	therefore, since $\J.\texttt{cnt}^{h}[u]=0$, 
	then $u$ is inconsistent \wrt $f^{\text{c}}\text{ in }\Gamma_{i^h, 1}$.

-- $u\in V_1$ and $\exists(v\in N^{\text{out}}(u))$ $(f^{\text{c}}(u)=f^{\text{c}}(v)=0$ 
		and $w(u,v)=i^h)$ (see line~\ref{subproc:repair:l3} of 
		$\texttt{repair}()$, SubProcedure~\ref{subproc:energy_jumps}). 
		In this case, $u$ is inconsistent \wrt $f^{\text{c}}\text{ in }\Gamma_{i^h, 1}$. Therefore, ${L^{\text{inc}}}^h\subseteq \text{Inc}(f^{\text{c}:h}, i^h, 1)$.
\begin{itemize}
\item ${L^{\text{inc}}}^h\supseteq \text{Inc}(f^{\text{c}:h}, i^h, 1)$:  
\end{itemize}
Fix $\hat{u}\in \text{Inc}(f^{\text{c}:h}, i^h, 1)$.
To begin, by (1.a), either $f^{\text{c}}(\hat{u})=0$ or $f^{\text{c}}(\hat{u})=\top$; 
since $\hat{u}\in \text{Inc}(f^{\text{c}:h}, i^h, 1)$, then $f^{\text{c}}(\hat{u})=0$. Still, 
by (1.b), $\hat{u}$ is consistent \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$.  
Let $(\hat{u},\hat{v})\in E$ be any arc which is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$.
\begin{itemize}
\item[If $\hat{u}\in V_0$, ] 
then, \emph{at least one} such a compatible  
$\hat{v}\in N^{\text{out}}(\hat{u})$ exists because $\hat{u}\in V_0$ is consistent 
\wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$. By (1.a), 
either $f^{\text{c}}(\hat{v})=0$ or $f^{\text{c}}(\hat{v})=\top$. 
Since $f^{\text{c}}(\hat{u})=0$ and 
$(\hat{u},\hat{v})$ is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$, 
then $f^{\text{c}}(\hat{v})=0$. Since $f^{\text{c}}(\hat{u})=f^{\text{c}}(\hat{v})=0$ and 
$\hat{u}\in \text{Inc}(f^{\text{c}:h}, i^h, 1)$, then $w(\hat{u},\hat{v})\leq i^h$.

We claim that at some step of execution of line~\ref{subproc:energy_jump:l3} 
in (the considered invocation of) $\texttt{ei-jump}()$ (SubProcedure~\ref{subproc:energy_jumps}), 
say at step $\iota'$ for $\iota < \iota' < h$, 
the entry $(w(\hat{u},\hat{v}), L_\alpha)$ is popped from $L_{\text{\bf{w}}}$.

-- If the considered invocation of $\texttt{ei-jump}(i,j)$ (at step $\iota$) 
is the very first one that is made by Algorithm~\ref{algo:solve_mpg}, then: $i=W^-$, 
and the front element of $L^{\iota}_{\text{\bf{w}}}$ is also $W^-$.
Therefore, since $W^-\leq w(\hat{u},\hat{v})\leq i^h$, 
at some step $\iota'$ for $\iota < \iota' < h$ as above, 
the entry $(w(\hat{u},\hat{v}), L_\alpha)$ is popped from $L_{\text{\bf{w}}}$.
 
-- If the current invocation of $\texttt{ei-jump}(i,j)$, 
at step $\iota$, is not the first made by Algorithm~\ref{algo:solve_mpg},
then $j\geq 2$ by Lemma~\ref{lem:ei-jump_state}. Since $f^{\text{c}}(\hat{u})=f^{\text{c}}(\hat{v})=0$, 
$j\geq 2$, and $(u,v)$ is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$, 
then $w(\hat{u},\hat{v}) > i$. By Lemma~\ref{lem:ei-jump_state}, 
when $\texttt{ei-jump}()$ is invoked (\ie at $\iota$), 
the front entry $(\bar{w}, L_{\bar\alpha})$ of $L^{\iota}_{\text{\bf{w}}}$ satisfies  
$\bar{w}=\min\{w_e\mid e\in E, w_e>i\}$. So, $\bar{w}\leq w(\hat{u},\hat{v})\leq i^h$. 
Thus, at some step of execution $\iota'$ for $\iota < \iota' < h$, 
the entry $(w(\hat{u},\hat{v}), L_\alpha)$ is popped from $L_{\text{\bf{w}}}$.

Soon after that $(w(\hat{u},\hat{v}), L_\alpha)$ have been popped from 
$L_{\text{\bf{w}}}$, then $\texttt{repair}(L_{\alpha}, \J)$ is invoked: 
there, since $f^{\text{c}}(\hat{u})=f^{\text{c}}(\hat{v})=0$ and $\hat{u}\in V_0$, 
then $\J.\texttt{cnt}[\hat{u}]$ is decremented by one unit at 
line~\ref{subproc:repair:l5} of $\texttt{repair}()$.

Indeed, this happens (after $\iota$ but within $\iota''$, \ie before $h$),  
\emph{for every} $v\in N^{\text{out}}(\hat{u})$ such that 
$(\hat{u}, v)\in E$ is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$. 
Thus, at $\iota''$, it holds that $\J.\texttt{cnt}^{\iota''}[\hat{u}]=0$, because \emph{all} of 
such $v\in N^{\text{out}}(\hat{u})$ had been visited by some invocation of 
$\texttt{repair}()$ (during the considered $\texttt{ei-jump}()$ 
that started at $\iota$), as described above. 
Then, $\hat{u}$ is inserted into $L^{\text{inc}}$; soon after, 
$\texttt{ei-jump}()$ halts (since $L^{\text{inc}}\neq\emptyset$); 
so, $\hat{u}\in {L^{\text{inc}}}^h$. Still, this holds for every $u\in \text{Inc}(f^{\text{c}:h}, i^h, 1)\cap V_0$; 
so, $\text{Inc}(f^{\text{c}:h}, i^h, 1)\cap V_0\subseteq  {L^{\text{inc}}}^h$.

\item[If $u\in V_1$, ] then, \emph{all} $\hat{v}\in N^{\text{out}}(\hat{u})$ are such that $(\hat{u}, 
\hat{v})$ is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$, 
because $\hat{u}\in V_1$ is consistent \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$. 
The argument proceeds almost in the same way as before, but of course quantifiers are interchanged.
By (1.a), either $f^{\text{c}}(\hat{v})=0$ or $f^{\text{c}}(\hat{v})=\top$. 
Since $f^{\text{c}}(\hat{u})=0$ and $(\hat{u},\hat{v})$ is compatible \wrt $f^{\text{c}}$ in $\Gamma_{i,j-1}$, 
then $f^{\text{c}}(\hat{v})=0$. Since $f^{\text{c}}(\hat{u})=f^{\text{c}}(\hat{v})=0$ and 
$\hat{u}\in \text{Inc}(f^{\text{c}:h}, i^h, 1)$, then $w(\hat{u},\hat{v})\leq i^h$.
By arguing as above, we see that at some step of execution of line~\ref{subproc:energy_jump:l3} 
in (the considered invocation of) $\texttt{ei-jump}()$ (SubProcedure~\ref{subproc:energy_jumps}), 
say at step $\iota'$ for $\iota < \iota' < h$, the entry $(w(\hat{u},\hat{v}), L_\alpha)$ 
is popped from $L_{\text{\bf{w}}}$. Soon after that $(w(\hat{u},\hat{v}), L_\alpha)$ have been popped from 
$L_{\text{\bf{w}}}$, then $\texttt{repair}(L_{\alpha}, \J)$ is invoked: 
there, since $f^{\text{c}}(\hat{u})=f^{\text{c}}(\hat{v})=0$ and $\hat{u}\in V_1$, 
then $\hat{u}$ is inserted into $L^{\text{inc}}$; soon after, 
$\texttt{ei-jump}()$ halts (since $L^{\text{inc}}\neq\emptyset$); 
so, $\hat{u}\in {L^{\text{inc}}}^h$. Still, this holds for every $u\in  \text{Inc}(f^{\text{c}:h}, i^h, 1) \cap V_1$; 
so, $ \text{Inc}(f^{\text{c}:h}, i^h, 1) \cap V_1\subseteq {L^{\text{inc}}}^h$.
\end{itemize} 
Therefore, $ \text{Inc}(f^{\text{c}:h}, i^h, 1) = {L^{\text{inc}}}^h$. 


